Visually Grounded Concept Composition

We investigate ways to compose complex concepts in texts from primitive ones while grounding them in images. We propose Concept and Relation Graph (CRG), which builds on top of constituency analysis and consists of recursively combined concepts with predicate functions. Meanwhile, we propose a concept composition neural network called Composer to leverage the CRG for visually grounded concept learning. Specifically, we learn the grounding of both primitive and all composed concepts by aligning them to images and show that learning to compose leads to more robust grounding results, measured in text-to-image matching accuracy. Notably, our model can model grounded concepts forming at both the finer-grained sentence level and the coarser-grained intermediate level (or word-level). Composer leads to pronounced improvement in matching accuracy when the evaluation data has significant compound divergence from the training data.

==> tables/full_coco_result.tex <==
%!TEX root = main.tex
\begin{table}[t]
    \centering
    \small
    {
        \tabcolsep 2pt
	    \begin{tabular}{@{\;} l@{\;\;} cc@{\quad} cc@{\;}}
	        \toprule
	        {} & \multicolumn{2}{c}{COCO$\rightarrow$COCO} &
	        \multicolumn{2}{c}{COCO$\rightarrow$F30K} \\
	        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
	        {Method}& {R1} & {R5} & {R1} & {R5} \\
	        \midrule
	        \VilMarker{} ViLBERT &  56.83 & 87.07 & \bf 46.62 & \bf 73.08 \\
	        \midrule
    	    \CMarker{} \ourmethod & \bf 59.40 & \bf 87.16 & 45.70 & 71.29 \\
	        \bottomrule
	    \end{tabular}
	}
	\caption{Image retrieval results of model trained on Full COCO training split.}
    \label{tab:full_coco}
\end{table}


==> tables/supp_flops_vs_composition_times.tex <==
%!TEX root = main.tex

\begin{table}[t]
    \centering
    \small
    \vspace{-1em}
    {
        \tabcolsep 2.5pt
	    \begin{tabular}{l@{\;} cccccc@{\;}}
	        \addlinespace
	        \toprule
	        {\# of Compositions} & &  2 & 3 & 4 & 5 \\
	        \midrule
	        {FLOPS} & &  38.37G & 38.40G & 38.44G & 38.47G\\
	        \bottomrule
	    \end{tabular}
	}
    \caption{FLOPS of \ourmethod under different number of compositions (The FLOPS calculate the FLOPS using the model with 6 layers of PT and 5 layers of CT)}
    \label{tab:supp_complexity_vs_num_composition}
\end{table}


